ALMA reveals thermal and non-thermal desorption of methanol ice in the HD 100546 protoplanetary disk

Methanol (CH$_3$OH) and formaldehyde (H$_2$CO) are chemically coupled organic molecules proposed to act as an intermediate step between simple molecules and more complex prebiotic compounds. Their abundance distributions across disks regulate the prebiotic potential of material at different disk radii. We present observations of multiple methanol and formaldehyde transitions toward the Herbig Ae disk HD 100546 obtained with ALMA, building upon the previous serendipitous detection of methanol in this source. We find that methanol has a higher rotational temperature ($T_\mathrm{rot}$) than formaldehyde towards both the centrally concentrated emission component in the inner disk ($0-110$ au) and a radially separate dust ring farther out in the disk ($180-260$ au). $T_\mathrm{rot}$ decreases for methanol and formaldehyde from the inner ($152^{+35}_{-27}$ K and $76^{+9}_{-8}$ K) to the outer disk ($52^{+8}_{-6}$ K and $31^{+2}_{-2}$ K), suggesting that we are tracing two different chemical environments. $T_\mathrm{rot}$ for both species in the inner disk is consistent with thermal desorption as the origin, while the outer disk reservoir is driven by non-thermal desorption. The CH$_3$OH/H$_2$CO column density ratio decreases from $14.6^{+5.2}_{-4.6}$ in the inner disk to $1.3^{+0.3}_{-0.2}$ in the outer disk, consistent with modelling predictions. The CH$_3$OH/H$_2$CO column density ratio for the inner disk is consistent with the median value in the range of column density ratios compiled from Solar System comets which would have formed at a similar distance. This supports the notion that interstellar ice is inherited and preserved by protoplanetary disks around solar-mass and intermediate-mass stars as we are seeing 'fresh' ice sublimation, as well as providing more evidence for the presence of prebiotic precursor molecules in planet-forming regions.

==> extra_text.tex <==
%A gas-grain chemical model of the HD 100546 disk predicts a similar decreasing trend in %the \ce{CH3OH}/\ce{H2CO} column density ratio with radius. 
%For the first time
%Therefore %particularly with methanol being the simplest example of a Complex Organic Molecule (COM). In this context, 
%a thorough molecular analysis of 
%the results from two observational datasets obtained towards % that consist overall of 13 methanol and five formaldehyde transitions. 
%This line-rich dataset enables us to % the actual results should go here
%(\ce{CH3OH}: $\sim 125-200$ H$_2$CO: $\sim$70-90 K) to the outer (CH$_3$OH: $\sim$45-60 K, H$_2$CO: $\sim$30 K) region. 
%abundance 
%Furthermore, 
%We also see a %similar 
%with a difference of an order of magnitude observed (inner: 14.6$^{+5.2}_{-4.6}$; outer: 1.3$^{+0.3}_{-0.2}$). 
%strongly suggest the presence of 
%A disk model 
%This supports the presence of 
%\textbf{hypothesis that} multiple desorption mechanisms 
%\textbf{exist} and therefore \textbf{there is} a radial difference in chemical environment, \textbf{including the local disk temperature and the distribution of large dust grains, which make up the bulk of the mass in the ice phase.} % a conclusion which affects the ongoing planet formation in this disk.
%, as well as to compare the CH$_3$OH/H$_2$CO ratios These are found to differ by an order of magnitude (inner: 12.1$^{+12.9}_{-6.2}$; outer: 1.72$^{+1.89}_{-0.85}$), reflecting opposing trends going from inner to outer component in the two molecules; we conclude that this is due to efficient gas-phase formation of H$_2$CO in the outer component. We also obtain find that the constrained rotational temperature measurements of both molecules significantly decreases from the inner region (130-160 K) to the outer region (30-40 K), We conclude that this is most likely reflecting a difference in ice desorption mechanism, with the low outer region temperature clearly indicating the icy nature of dust grains here. 
%\twocolumn
% \citealt{Bergman2011}%\citealt{Roberts2007}, %\citealt{Menten1988}, %the early 
%,Santos2022 stages of stellar formation
%\rm{CO + H \rightarrow  H_2CO}
%and simulated chemical modelling research
%taking astrochemical inventory of objects in the later stages of low-mass stellar system formation is in its infancy relative to studies of older objects. 
%This is due to the small angular size of protoplanetary disks, which are on the scale of approximately hundreds of au, 
%at least an order of magnitude smaller than objects undergoing earlier stages of star formation (see \citealt{Nakamoto1994} and references therein) and thus requiring higher spatial resolution to observe. 
%Consequently, until recently, the chemical study of these objects and the potential resultant glimpse into the chemical environment in which planets form has remained hypothetical. 
%life-supporting COMs 
%as a result of a dedicated study
%an object with sufficiently low temperatures for CH$_3$OH ice formation 
% surrounding a T Tauri star
%be more hostile and survival 
% seemingly explaining the supposed absence.
%In situ formation of the simplest COM from a CH$_3$OH ice reservoir is ruled out in HD 100546 due to the warm disk temperature, leading to the conclusion that gas phase CH$_3$OH in the HD 100546 disk has been inherited from previous star formation stages. This finding therefore suggests that an organic molecule that is a precursor for prebiotic molecules survives the disk formation process and is therefore available during the planet formation process. Moreover, two distinct emission components were detected, one being centrally concentrated with the other coincident with the previously \textbf{tentatively} detected dust ring at approximately 200 au, giving rise to the possibility that two distinct desorption mechanisms are at play in this disk, which may be a result of two distinct temperatures. This is one line of investigation that is explored in the present work. 
%, which may be a result of two distinct temperatures
%The source targeted, HD 100546, is also the subject of this work, although 
%and/or exposure to high temperature %, towards HD 100546, obtained with an improved beamsize giving rise to an angular resolution of approximately 33 au. 
%Through rotational diagram analysis, we aim to constrain the temperature of the two distinct CH$_3$OH emission components in an attempt to discern the particular desorption mechanism(s) at play for this unexpected gas phase emission. In addition, we present in this work supplementary Cycle 7 observations of CH$_3$OH and H$_2$CO, %In addition to its coupled formation mechanism, H$_2$CO is relevant because previous research has shown that low CH$_3$OH/H$_2$CO ratios are associated with chemical processing of accreting material in disks and/or with temperature (\citealt{vantHoff2020}, \citealt{Podio2020}). This supplementary data also 
%enabling a rotational diagram analysis of H$_2$CO to also be completed, constraining the rotational temperature and column density of this molecule in this source and facilitating comparison with CH$_3$OH. 
%The CH$_3$OH observations towards HD 100546, along with observations of H$_2$CO, are presented and analysed in this work. 
%including H$_2$CO and CH$_3$OH (the focus of this work), the more complex CH$_3$OCHO, another species that is important in building life-sustaining molecules, as well as, for the first time in a protoplanetary disk, the isotopologues H$^{13}_2$CO and $^{34}$SO.
%, along with CH$_3$OH towards both. 
% You should avoid orphan sub-sections - I've moved some of this to the next section
%It is in this context that 
%In theory, however, the warmer temperature of disk due to the influence of the Herbig Ae/Be star would prevent the ice phase formation of more complex molecules, including COMs. Nevertheless, gas phase CH$_3$OH has been serendipitously detected towards this disk by \citet{Booth2021} using ALMA Cycle 7 observations with a beamsize of 1.40" $\times$ 1.11". However, due to the limitations presented by the angular resolution of these observations, the particular desorption mechanism(s) at play could not be determined.
%In order to investigate HD 100546 in more detail, including the desorption mechanisms at play in the separate components, 
%These observations form part of a larger dataset from an ALMA program targeting multiple molecules towards the Herbig disks HD 100546 and IRS 48 (program 2021.1.00738.S, PI: A. S. Booth; see \citealt{Booth2024HD}, \citeyear{Booth2024IRS} for further details). 
% Put this in the acknowledgements
%\footnote{CASA is developed by an international consortium of scientists based at the National Radio Astronomical Observatory (NRAO), the European Southern Observatory (ESO), the National Astronomical Observatory of Japan (NAOJ), the Academia Sinica Institute of Astronomy and Astrophysics (ASIAA), the CSIRO division for Astronomy and Space Science (CASS) and the Netherlands Institute for Radio Astronomy (ASTRON) under the guidance of NRAO.}
%has been applied to all images presented in this paper in order to boost the weak signal-to-noise ratio (s/n) of the CH$_3$OH lines detected. 

%We use only the lines that are sufficiently well separated enough to be included in our analysis are included in Table \ref{table.trans}
% \ce{CH$_3$OH and 
%(refer to \citealt{Booth2021}, \citeyear{Booth2023a} for further details).
% while the spectral resolution is 0.25 km~s$^{-1}$. The cleaning process is the same as described above for the Cycle 8 lines; in addition, we convolve this data to match the 0.3" beamsize of the Cycle 8 observations. 
%two of CH$_3$OH lines detected in the Cycle 8 observations at 338.513 GHz are blended with each other, while another the CH$_3$OH line at 350.688 GHz is blended with a line of NO at 350.689 GHz}. Blending also affects 
%To aid comparison, all Cycle 7 images were convolved to match the Cycle 8 beamsize for the analyses described in Sect. \ref{Methodology}.
% convolved with a circular beam of Full Width at Half Maximum (FWHM) 1"

%Due to the spatial resolution of our observations being sufficient to resolve radially varying linewidths, the mask utilises the power law described in Eq. \ref{eq.kepmask} as a radial profile. 
%In this equation, $\Delta$V$_0$ is the linewidth at 1" and the exponent of the power law is represented by $\Delta$V$_q$; for our mask these values have been optimised by eye at 200 m~s$^{-1}$ and -0.5, respectively.
%\begin{equation}
%    \Delta V(r)=\Delta V_0\times \Bigg(\frac{r}{1"}\Bigg)^{\Delta V_q}
%    \label{eq.kepmask}
%\end{equation}
%    \caption{E$_u$ and A$_{ul}$ taken from LAMDA. g$_u$ and E$_l$ taken from CDMS.}
%    \centering
%\begin{figure*}[hbt!]
 %   \centering
    
  %  \caption{Spectral line profiles for all ten detected \ce{CH3OH} lines extracted using \texttt{gofish} in order of ascending $E_\mathrm{u}$ values.
   % These spectral lines have been generated by integrating the emission between 0 and 110 au for the full velocity range of -4.2 and 17.4 km~s$^{-1}$. 
    %The dashed line represents the $v_\mathrm{LSR}$ of this source (5.7 km~s$^{-1}$).}
    %\label{fig.gofish_wide}
%\end{figure*}

%The inner component is bright in the highest energy \ce{H2CO} line ($E_\mathrm{u} = 140.9$~K), while the outer ring of emission is brightest in the lowest energy \ce{H2CO} line ($E_\mathrm{u} = 62.5$~K).
%Similarly, we see the same signature in the \ce{CH3OH} emission. 
%, showing both emission components.
%    \caption{Upper row (left to right): 0.9 continuum dust emission first published in \citealt{Booth2024HD}, plotted in log scale in order to exaggerate the outer ring continuum emission; stacked moment 0 map consisting of combining our 10 detected CH$_3$OH lines% (we exclude the line that is blended with a transition of NO)
%    , stacked moment 0 maps consisting of combining only the lines in our sample with visible outer ring emission with a stretched scale in which the midpoint is at 8 mJy~beam$^{-1}$ in order to improve the ring emission visibility. Lower row (left to right): Moment 0 maps showing H$_2$CO lines from coldest %(5$_{1,5}$-4$_{1,4}$ at 62.5 K) 
%    to hottest% (4$_{3,2}$-3$_{3,1}$
%    . }
%Fig. \ref{fig.morph} shows the continuum image of HD 100546 (first published in \citealt{Booth2024HD}) compared to moment 0 maps for the coldest (5$_{1,5}$-4$_{1,4}$ at 62.5 K) and hottest (4$_{3,2}$-3$_{3,1}$ and 4$_{3,1}$-3$_{3,0}$ at 140.9 K) lines of H$_2$CO along with stacked maps of CH$_3$OH. We also compare in this figure two stacked moment 0 maps, one consisting of all lines of CH$_3$OH in our sample %(excluding the line at 350.688 GHz which, as will be detailed in Sect. \ref{Methodology}, was later found to be blended with a line of NO at 350.689 GHz)
%and the other consisting of the four lines with the lowest E$_u$ values, which, according to the azimuthally averaged radial profiles shown in Fig. \ref{fig.azavouter}, show signs of outer ring emission at approximately 200 au in addition to the centrally concentrated emission component detected in all CH$_3$OH lines (azimuthally averaged radial profiles for all CH$_3$OH lines in our sample can be found in the Appendix). Note that outer ring emission was also detected in a fifth CH$_3$OH line at 350.688 GHz, however, this line is affected by blending due to the presence of a line of NO at 350.689 GHz and is therefore not included.

%Fig. \ref{fig.azav_H2CO} shows azimuthally averaged radial profiles for the H$_2$CO lines in our sample. Note that while Table \ref{table.trans} lists five H$_2$CO lines, we only show four radial profiles. This is due to the close proximity of the two H$_2$CO lines detected at approximately 291.38 GHz in Cycle 7 which puts them in the same spw as one another; as a result, this radial profile contains contributions from both blended lines.
%    The Cycle 7 data in the rightmost three panels have been convolved to the same beamsize as the Cycle 8 data in the left panel. 

%\begin{figure*}[hbt!]
 %   \centering
    
  %  \caption{Azimuthally-averaged radial profiles for the \ce{H2CO} lines in order of descending peak intensity. 
   % The two dust rings seen in the 0.9 mm continuum emission at $\sim$20 au and $\sim$200 au are denoted by the dashed vertical lines. 
    %The horizontal bar shows the semi-major axis of the beam.}
    %\label{fig.azav_H2CO}
%\end{figure*}

%\subsection{Cycle 7}
%Figs. \ref{fig.radprof} and \ref{fig.mom0_maps} show the moment 0 maps and radial profiles, respectively, for the CH$_3$OH, p-H$_2$CO and o-H$_2$CO emission detected using the Cycle 7 observations. It is clear from these maps that we detect both previously identified components - one that is centrally concentrated and the other forming a ring at $\sim$~200 au - in both formaldehyde and methanol. It is also clear that the signal-to-noise ratio (s/n) for the p-H$_2$CO transition is much lower than for the CH$_3$OH and o-H$_2$CO transition, which is expected given the o-p ratio of formaldehyde in this environment (citation?).
%\\
%\\
%\subsection{Cycle 8}
%We also show in Fig. \ref{fig.stackedmom0} the moment 0 map generated from the channel map in Fig. \ref{fig.stackedchan} in the Appendix, which was created by stacking the channel maps of the individual spws for the 12 CH$_3$OH lines in our Cycle 8 sample. which can also be found in the Appendix (Figs. \ref{fig.firstchan} to \ref{fig.lastchan}).
%\\
%\\
%Another clear observation that can be taken from the individual channel maps of the Cycle 8 CH$_3$OH transitions is the relative absence of the outer emission component. Emission corresponding to the previously detected mm dust ring at approximately 200 au (\citealt{Walsh2014}) is visible in only two transitions: those at 338.408 GHz and 338.345 GHz, which have E$_u$ values of 65 K and 71 K, respectively. This is an insufficient range of E$_u$ to perform a rotational diagram analysis. A comparison between the column density and rotational temperature values measured towards these two radially separate components is, therefore, not possible with our current data. However, a constrained rotational temperature towards the inner component within approximately 110 au, corresponding to the planet-forming region of this source, is achievable due to the clear detection of this component towards all 12 lines, which will still probe the hypothesis that CH$_3$OH is inherited in this source (\citealt{Booth2021}).
% 
%The propagated uncertainty for S$_\nu\Delta$v using the GoFish extracted flux density \textbf{statistical} uncertainties were \textbf{likely to be} an underestimation. 
% extracted using both GoFish and Specflux%We note here that, due to the presence of two fully blended \ce{H2CO} lines with identical A$_{ul}$, g$_u$ and E$_u$ values, in this case we measure the total flux across both blended lines and quote the individual values assuming an equal contribution from both. 
%, meaning the linewidths are not properly corrected for Keplerian rotation; GoFish is optimised to extract the flux of spatially resolved lines assuming a disk-averaged spectrum using the \textit{integrated\_spectrum} tool and so there is the potential for inaccuracies here. 

%In order to check the suitability of GoFish for extraction in our case of unresolved emission, we also performed an identical flux extraction and eventual rotational diagram analysis using Specflux within CASA, which returns accurate flux extraction values even in the case of spatially unresolved lines. We run Specflux using an elliptical aperture of 1" to match the 110 au extent of the GoFish extraction (covering the inner region where emission is seen in all cases). We find that both methods return the same results for integrated flux density and rotational temperature, thus validating our use of GoFish for our whole analysis. \textbf{The lower panel of} Fig. \ref{fig.ch3oh_outer_spec} shows the extracted spectra using GoFish for all CH$_3$OH transitions observed in the inner disk. 
%are then used to calculate the total integrated flux density using the rectangle rule to integrate, such that:
%\begin{equation}
%\rm{S_\nu}\Delta\rm{v}=\Sigma^n_{i=1}\Delta\rm{v} F_n,
%\label{eq.integration}
%\end{equation}
%where \textit{F} represents the extracted flux density values in mJy~km~s$^{-1}$ and \textit{n} is the total number of flux density values extracted. 
%extrusing \texttt{gofish} with a velocity clip between -0.6 and 12.0 km~s$^{-1}$ for the inner region extraction and between approximately 4.5 and 6.9 km~s$^{-1}$ for the outer region extraction (unless otherwise noted), along with column density values calculated using Eq. \ref{eq.nu} for all lines in our sample
%. We also include opacity measurements for the lines that are included in the rotational diagram analysis.%$^{(b)}$The outer H$_2$CO analysis had a tighter velocity clip between 2.0 and 8.0 km~s$^{-1}$ due to narrower linewidths (with one exception, refer to note $^{(d)}$)\\ %$^{(e)}$Two CH$_3$OH lines are blended, as mentioned in Section \ref{Observations}, therefore they are measured assuming an equal contribution from both lines to the extracted flux    %, with the exception of the line at 350.905 GHz which is blended with a line of NO
%;  therefore assumes a 1:1 ratio between these S$_\nu\Delta$v values. %with higher redshift/blueshift components possibly tracing a disk wind or outflow; the other explanation is that there are other non-CH$_3$OH lines present in these spws. 
%However, hence, to extract the line fluxes for each line, we applied a velocity
%necessitating the velocity clipping used in our analysis such that the CH$_3$OH data used is not contaminated in any way. %These contaminant lines are also visible in some of the channel maps shown in the Appendix. 
%Regardless, referring to the spectra shown in Fig. \ref{fig.ch3oh_outer_spec}, we \textbf{therefore} apply a velocity clip ranging from %Figs. \ref{fig.radprof8} and \ref{fig.mom0_cycle8}, which show respectively, the moment 0 maps and radial profiles for the CH$_3$OH emission detected in HD 100546 from the Cycle 8 observations, have been generated from data clipped to a velocity range of 
 %We further discuss the contaminant lines in Section \ref{contaminated_lines}.
%For the \ce{H2CO} lines, we match the velocity clip used in the inner and (in most cases) outer region extraction to those used for CH$_3$OH in order to facilitate comparison as the linewidths are similar. 
%However, as previously mentioned, ; due to the difference in linewidth between detections towards the inner and outer regions, this is sufficient to appear blended in the spectrum extracted for the inner region (see Fig. \ref{fig.h2co_inner_spec}) but well separated in the spectrum extracted for the outer region (see Fig. \ref{fig.h2co_outer_spec}). In order to account for this, we extract the lines in the inner region using the same velocity clip as all other lines (-0.6 to 12.0 km~s$^{-1}$), which covers both blended lines. Referring to Table \ref{table.trans},  A velocity clip between 4.5 and 6.9 km~s$^{-1}$ was applied to the Cycle 8 H$_2$CO line for outer region extraction in order to match that used for the Cycle 8 CH$_3$OH outer region extraction; this velocity clip was also utilised for the extraction of the line at 291.238 GHz, while a slightly adjusted velocity clip between 4.6 and 6.5 km~s$^{-1}$ was applied to the line at 291.948 GHz due to a slightly narrower linewidth. Thus, we are able to extract flux separately from both the inner and outer emission components seen in HD 100546 for both molecules.

% This is overexplained, I've reduced it down
%Therefore, for the inner region flux extraction, the \textit{r} value in Eq. \ref{eq.omega} is 110 au, while for the outer region flux extraction, we calculate $\Omega$ as the difference between the solid angle as calculated using Eq. \ref{eq.omega} assuming an \textit{r} value of 260 au and that assuming an \textit{r} value of 180 au. This leads to $\Omega$ values of 7$\times$10$^{-11}$ sr for the inner region and 2$\times$10$^{-10}$ sr for the outer region. 

%Through error propagation of Eq. \ref{eq.omega}, the uncertainty in $\Omega$ is therefore calculated using the following equation:
%\begin{equation}
%\Delta\Omega=\Omega\pi\sqrt{\frac{2\Delta r}{r}^2+\frac{2\Delta d}{d}^2}.
%\label{eq.deltaomega}
%\end{equation}
%As can be seen in Figs. \ref{fig.azavouter} and \ref{fig.azav_H2CO} (refer also to Fig. \ref{fig.radprof8} in the Appendix), four out of the 10 well separated CH$_3$OH lines in our sample, as well as all four H$_2$CO lines, show evidence of an outer emission component between approximately 180-260 au,%. It should be noted that these four lines have the lowest E$_u$ values across the sample; 
%Comparing the spectral profiles for the outer region shown in Fig. \ref{fig.ch3oh_outer_spec} to those for the inner region in Fig. \ref{fig.gofish_wide}, the outer region lines have very narrow linewidths
%, although the line at 350.688 GHz is slightly broader. Upon investigation, this broader linewidth is due to the presence of a transition of NO at 350.689 which is blended with this CH$_3$OH line. As a result of this, we will be fully removing this CH$_3$OH line from our analysis. Meanwhile, the H$_2$CO radial profiles shown in Fig. \ref{fig.azav_H2CO} also show evidence of outer ring emission at a similar distance. This 180-260 au range is 
%therefore we run the flux extraction using this radial range in order to complete the rotational diagram analysis for the outer region. 
%, with the error propagated accordingly

%We also note that the ALMA dataset obtained towards HD 100546 is very line-rich, so much so that some of the spws that we target to detect our CH$_3$OH lines are also covering frequencies where we detect emission that is well separated from the target CH$_3$OH line frequency. We explore the potential origins of this emission in Sect. \ref{Discussion} but, regardless, this presents a potential contamination issue for our analysis. As a result of this, as well as to avoid including any line-free channels in our analysis, we have applied a velocity clip to our CH$_3$OH observations.
%we originally planned to run this analysis with different aperture values. However, it is clear from both the radial profiles in Fig. \ref{fig.radprof8} and the channel maps shown in the Appendix that emission outside the centrally concentrated component is only detected in two transitions: 7$_{0,7}$-6$_{0,6}$ at 338.408 GHz and 7$_{1,7}$-6$_{1,6}$ at 338.345 GHz. As can be seen in Table \ref{table.trans}, the spread in E$_u$ between these two transitions is only $\sim$6 K, thus we cannot constrain the temperature in the outer component using a rotational diagram analysis. We do, however, clearly detect emission in the inner component in all 12 transitions considered, therefore the rotational diagram analysis can be used to constrain the temperature here. We therefore choose the radial extent to match the aperture that we are considering for the inner region, which is 110 au. %(investigating the centrally concentrated emission component), 440 au for the total region (investigating the disk as a whole) and the difference ($\Omega_{TOT}$-$\Omega_{IN}$) for the outer region (investigating the ring emission component). 
%, (1.1 $\pm$ 0.1)$\times$10$^{-9}$ sr for the outer region and (1.2 $\pm$ 0.1)$\times$10$^{-9}$ sr for the total region. 
%Meanwhile, in order to compute the integrated flux density, we must first extract the flux from our inner region. Due to weak s/n in some cases, however, not all of the lines are spatially resolved. 
% the inner disk component is unresolved


%Note that the velocity range of these spectra is -4.2 to 17.4 km~s$^{-1}$, which represents the full spw. However, for the rotational diagram analysis we clip this velocity range to -0.6 to 12.0 km~s$^{-1}$.
%The spectra extracted using Specflux can be found in Fig. \ref{fig.specflux_wide} in the Appendix. % in Cycles 7 and 8.
%\begin{figure}
 %   \centering
  %  \includegraphics[width=0.45\textwidth]{images/spectra_gofish.png}
   % \caption{FIX THIS CAPTION Flux extracted from the 11 Cycle 8 CH$_3$OH transitions. From left to right: spectra extracted using Specflux with an elliptical mask of aperture 110 au, matching the extent of the centrally concentrated emission component; spectra extracted using GoFish with an aperture of 110 au,; spectra extracted using GoFish for the whole disk excluding the inner 110 au, covering the area where the ring emission component is seen; spectra extracted using GoFish with an aperture of 440 au, covering the extent of the full disk emission. The y axes of the two leftmost and two rightmost columns are shared to facilitate comparison.}
    %\label{fig.spectra}
%\end{figure}

%As such, error propagation dictates that the uncertainty in our values for S$_\nu\Delta~$v is calculated using the following equation:
%\begin{equation}
%\Delta S_\nu\Delta\rm{v}=\Delta\rm{v}\sqrt{\Delta F_1^2+\Delta F_2^2+...+\Delta F_n^2}.
%\label{eq.uncertaintyintegratedfluxdensity}
%\end{equation}
\\
\\
%Referring to Eq. \ref{eq.nu},% with $\Omega$ and S$_\nu\Delta\rm{v}$ being the only parameters with associated uncertainties,
%the following equation is used to calculate the uncertainty in the column density values:
%\begin{equation}
%\Delta N_u^{thin}=N_u^{thin}{\frac{\Delta S_\nu\rm{v}}{S_\nu\rm{v}}}.
%\label{eq.deltanu}
%\end{equation}
%Using the Boltzmann distribution, one can write Eq. \ref{eq.nu} to relate the column density in the upper energy level, N$_u^{thin}$, to the total column density, N$_T$ (cm$^{-2}$):
%\begin{equation}
%   \frac{N_u}{g_u}=\frac{N_T}{Q(T_{rot})}e^{-\frac{E_u}{k_BT_{rot}}},
%   \label{eq.nugu}
%\end{equation}
%where g$_u$ represents the upper level degeneracy, E$_u$ is the energy of the upper level (K), T$_{rot}$ is the rotational temperature (K), Q(T$_{rot}$) is the partition function at this temperature and k$_B$ is the Boltzmann constant in cgs units. Where available, the partition function values are taken from CDMS. 
%For temperatures above those for which partition function values are available on CDMS, we calculate these values using the high temperature approximation, which can be expressed as follows:
%\begin{equation}
%    Q(T_{rot})=\frac{\sqrt{\pi}}{\sigma}\sqrt{\frac{(k_BT)^3}{ABCh^3}},
%    \label{eq.partitionfunction}
%\end{equation}
%where $\sigma$ represents the rotational symmetry number and A, B and C represent rotational constants (MHz) of the relevant molecule, which are obtained from CDMS.
%Table \ref{tab.qrot} shows the values of Q(T$_{rot}$) assuming temperature values of 50 K, 100 K, 150 K and 200 K.
%\begin{table}[hbt!]
 %   \centering
  %  \caption{Partition function values, interpolated using data from CDMS, for H$_2$CO and CH$_3$OH at the four aforementioned T$_{rot}$ values.}
   % \begin{tabular}{c c c c c}
    %& & & & \\
     %   \hline
      %   Molecule & & Q(T$_{rot}$) & & \\
       %  & 50 K & 100 K & 150 K & 200 K \\
        % \hline
         %& & & & \\
         %H$_2$CO & 182 & 511 & 1020 & 1529 \\
         %& & & & \\
         %CH$_3$OH & 1354 & 4369 & 9750 & 16507 \\
         %& & & & \\
         %\hline
    %\end{tabular}
    %\label{tab.qrot}
%\end{table}
%Taking the logarithmic of Eq. \ref{eq.nugu} results in Eq. \ref{eq.log}:
%\begin{equation}
%    ln\frac{N_u^{thin}}{g_u}=ln~N_T - ln~Q(T_{rot}) - \frac{E_u}{k_BT_{rot}}.
%    \label{eq.log}
%\end{equation}
%From this equation, through plotting a rotational diagram ($\frac{N_u^{thin}}{g_u}$ vs E$_u$), one can deduce T$_{rot}$ and N$_T$ from the gradient and intercept, respectively. In order to achieve this, we utilise an MCMC procedure first published in \textbf{\citet{Loomis2018}} using our measured S$_\nu\Delta$v values as input values.
\\
\\
%\subsection{H$_2$CO blended lines}
%Although there are five lines in our H$_2$CO sample, the Cycle 7 data contains two pairs of lines, one p-H$_2$CO and one o-H$_2$CO, that have the same E$_u$ value as each other, therefore only three separate E$_u$ values are represented by our H$_2$CO dataset% and thus would be a single point on a rotational diagram
%. The p-H$_2$CO pair of lines are well separated and in separate spws and are therefore analysed as explained previously for other lines. However the o-H$_2$CO pair of lines at 291.38 GHz appear in the same spw at a separation of approximately 5 km~s$^{-1}$. Referring to Figs. \ref{fig.h2co_inner_spec} and \ref{fig.h2co_outer_spec} in the Appendix, it is clear that these o-H$_2$CO lines are blended in the inner component but well separated in the outer component. We checked how stacking each pair of lines would affect our results but the aforementioned assumption of 10\% flux uncertainty remains dominant.
%\\
%\\
%Consequently, for the purpose of our rotational diagram analysis, we %include one H$_2$CO line for each E$_u$ value, as denoted in Table \ref{table.rotdiagtrans}. However, despite being well separated in velocity, the two o-H$_2$CO lines in Cycle 7 appear in the same spw within the velocity clip used for CH$_3$OH. We 
%investigated how applying a tighter velocity clip of 2.0 to 8.0 km~s$^{-1}$ across all H$_2$CO lines would affected our results, as this would take into account only one of the o-H$_2$CO lines according to the spectrum for the outer region shown in Fig. \ref{fig.h2co_outer_spec}. For the inner region, the values were within uncertainty of those obtained with the wider velocity clip, although due to the wider linewidth of the Cycle 8 H$_2$CO line some flux was cut off (refer to Fig. \ref{fig.h2co_inner_spec} in the Appendix). However, for the outer region, the effect of reducing the velocity clip on the amount of flux extracted from the Cycle 7 lines was profound. As a result of this, as well as the fact that no flux was lost from the Cycle 8 line as a result of reducing the velocity clip range due to ubiquitously narrower linewidths in the outer region, a tighter velocity clip between 2.0 and 8.0 km~s$^{-1}$ is applied to the outer region extraction only for all H$_2$CO lines, while for all H$_2$CO lines, with the exception of the o-H$_2$CO lines at 291.38 GHz, the inner region extraction had a velocity clip of -0.6 to 12.0 km~s$^{-1}$ to ensure that no flux was lost from the Cycle 8 line and also to match the velocity clip used for the CH$_3$OH rotational diagram analysis. 
%\\
%\\
%In the case of the o-H$_2$CO lines, the reduced velocity clip applied to the outer region therefore, by design, measures the flux of the line at 291.384 GHz only, as the line at 291.380 GHz is cut off by the reduced velocity clip. We therefore also run the flux extraction of this same spw with a velocity clip of 8.0 to 11.0 km~s$^{-1}$ in order to separately measure the flux extracted from the outer region for the line at 291.380 GHz. For the inner region, where the o-H$_2$CO lines are blended, the wider velocity clip between -0.6 to 12.0 km~s$^{-1}$ therefore extracts flux from both lines. Similarly to the blended CH$_3$OH transitions at 338.513 GHz, these H$_2$CO lines have equal A$_{ul}$, E$_{u}$ values and g$_{u}$ values and so we can safely assume that they will have an equal contribution to the total flux extracted from the inner region using the wider velocity clip. The S$_\nu\Delta$v values for these o-H$_2$CO lines in the inner regions quoted in Table \ref{table.rotdiagtrans} therefore takes this assumption into consideration. 
%\\
%\\
%To avoid contamination, %Keplerian masks for each line were created using a dedicated script (citation) and it was determined that emission of the target CH$_3$OH line is only seen between -0.6 and 12 km s$^{-1}$. Thus, when extracting flux using GoFish, 
%we clip the velocity to a range which only takes into account the CH$_3$OH emission: -4.2 to 17.4 km~s$^{-1}$, matching the data used to generate the radial profiles and moment 0 maps shown in Figs. \ref{fig.radprof8} and \ref{fig.mom0_cycle8}, respectively. 
%Fig. \ref{fig.gofish_wide} show spectra extracted from our 12 CH$_3$OH transitions using GoFish. 
%; the more narrow range contains only CH$_3$OH emission according to the channel maps of stronger lines with no possibility of contamination but the wider range was employed to take into account possible broader features seen in weaker lines.
%\begin{figure*}
 %   \centering
  %  \includegraphics[width=0.8\textwidth]{images/mask_check_specflux_flux.png}
   % \caption{Flux extracted from Keplerian masks generated with target resolutions of 1.0" (upper row) and 2.0" (lower row) for each targeted CH$_3$OH transition. The total integrated flux is shown above each panel.}
    %\label{fig.kep_spectra}
%\end{figure*}
%\\
%\\
%to be potentially edited following search for more lines
%\\Due to the wide range of upper energy values covered by our sample of CH$_3$OH lines (refer to Table \ref{table.trans}), only some of the lines are detected with sufficiently high signal-to-noise ratio (s/n) to be spatially resolved. As a result of the shift and stack method employed by GoFish during flux extraction, signal is therefore only extracted in these cases. %As a result, this method of flux extraction cannot be used for all of the lines in our sample. For those lines that are spatially unresolved, a different method of flux extraction is required to obtain the signal - \textit{specflux} in CASA is more suitable in these cases. In order to optimise the aperture size used to extract flux using \textit{specflux}, we compare flux extracted from the weakest line - 13(0,13)-12(1,12) - with aperture sizes of 1", 2", 3" and 4"; as can be seen in Figure \ref{fig.ellipse_comparison}, 1" is the only case in which flux signal was extracted as this resulted in the only positive value for total integrated flux.
%Therefore, flux was extracted using GoFish for the following lines (strongest to weakest): 7(0,7)-6(0,6), ... . Flux was extracted using \textit{specflux} for the following lines (strongest to weakest): ... and 13(0,13)-12(1,12).}
%\begin{figure}
 %   \centering
  %  \includegraphics[width=0.5\textwidth]{images/test_weak_specflux_ellipse_comparison.png}
   % \label{fig.ellipse_comparison}
%\end{figure}
%Given the weak s/n ratio of some of the CH$_3$OH lines in our Cycle 8 sample and in an attempt to define a threshold for usable lines, we investigated the filter response (refer to Booth et al. in prep.) using a mask with a radius of 100 au and, as a result, determined that using 6$\sigma$ as a filter response threshold enabled only lines with clearly detected spatially resolved emission to be included in the rotational diagram analysis. It should be noted that CH$_3$OH lines at approximately 338.5 GHz and 338.7 GHz are predicted to have responses above this threshold, however, these are not included in our sample because there are multiple lines at 338.5 GHz that are affected by blending and because the line at 388.7 GHz is not detected. Additionally, note that the line at 350.688 GHz is blended with a line of NO at 350.689 GHz and is therefore not included in our analysis. Table \ref{table.rotdiagtrans} shows the values of the parameters required for the rotational diagram analysis using the Cycle 8 CH$_3$OH transitions which meet this filter response threshold.
%\begin{table*}
%    \tiny
 %   \centering
  %  \caption{Total (0-440 au), Inner (0-110 au) and Outer (110-440 au) flux measurements extracted using GoFish (GF), Specflux using a Keplerian mask with target resolutions of 1.0" (Kep 1.0") and 2.0" (Kep 2.0"), as well as Specflux using an elliptical mask (Ellipse). A velocity clip between -0.6 and 12 km~s$^{-1}$ has been applied to the extractions using GoFish and Specflux with an elliptical mask.}
   %     \resizebox{\textwidth}{!}{\begin{tabular}{c c c c c c c c c c c c c}
    %         & & & & & & & & & & & & \\
     %        \hline
      %       Frequency [GHz] & \multicolumn{4}{c}{S$_\nu\Delta$v$_{TOT}$ [mJy~km~s$^{-1}$]} & \multicolumn{4}{c}{S$_\nu\Delta$v$_{INN}$ [mJy~km~s$^{-1}$]} & \multicolumn{4}{c}{S$_\nu\Delta$v$_{OUT}$ [mJy~km~s$^{-1}$]} \\
       %      \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
        %     & GF & Kep 1.0" & Kep 2.0" & Ellipse & GF & Kep 1.0" & Kep 2.0" & Ellipse & GF & Kep 1.0" & Kep 2.0" & Ellipse \\
         %    \hline
          %   & & & & & & & & & & & & \\
           %  338.408 & 213.81 $\pm$ 32.66 & 244.44 $\pm$ 14.43 & 200.19 $\pm$ 14.43 & 146.45 $\pm$ 14.43 & 128.01 $\pm$ 7.36 & 140.91 $\pm$ 14.43 & 116.33 $\pm$ 14.43 & 146.45 $\pm$ 14.43 & 158.93 $\pm$ 31.09 & 103.53 $\pm$ 14.43 & 83.87 $\pm$ 14.43 & 0.00 $\pm$ 14.43 \\
            % 338.345 & 185.26 $\pm$ 33.62 & 194.24 $\pm$ 51.89 & 140.23 $\pm$ 51.89 & 118.40 $\pm$ 51.89 & 89.76 $\pm$ 6.03 & 94.82 $\pm$ 51.89 & 75.33 $\pm$ 51.89 & 112.22 $\pm$ 51.89 & 197.04 $\pm$ 32.19 & 99.43 $\pm$ 51.89 & 64.90 $\pm$ 51.89 & 6.18 $\pm$ 51.89 \\
             %338.124 & 151.68 $\pm$ 32.90 & 162.48 $\pm$ 4.32 & 154.79 $\pm$ 4.32 & 151.43 $\pm$ 4.32 & 98.09 $\pm$ 6.12 & 101.63 $\pm$ 4.32 & 100.71 $\pm$ 4.32 & 96.35 $\pm$ 4.32 & 144.49 $\pm$ 31.49 & 60.85 $\pm$ 4.32 & 54.08 $\pm$ 4.32 & 55.08 $\pm$ 4.32 \\
             %338.614 & 98.76 $\pm$ 31.28 & 96.39 $\pm$ 23.16 & 95.30 $\pm$ 23.16 & 114.31 $\pm$ 23.16 & 102.54 $\pm$ 5.86 & 95.59 $\pm$ 23.16 & 92.45 $\pm$ 23.16 & 117.08 $\pm$ 23.16 & 96.98 $\pm$ 29.96 & 0.80 $\pm$ 23.16 & 2.85 $\pm$ 23.16 & 0.00 $\pm$ 23.16 \\
            % & & & & & & & & & & & & \\
            % \hline
        %\end{tabular}}
%\end{table*}
%\subsection{Cycle 7}
%\begin{table*}
 %   \small
 %   \centering
 %   \caption{Total, Inner (0-150au) and Outer (150-200au) integrated flux densities measurements for Cycle 7 p-H$_2$CO, o-H$_2$CO and CH$_3$OH transitions extracted using GoFish, radial emission extent obtained from data, column density calculated using Eq. \ref{eq.nu} and other values taken from CDMS and LAMDA. For now only robust 2.0 values are included as the 0.5 struggles more to detect the lines in the outer disk.}
  %  \begin{tabular}{c c c c c c c c c c}
  %      & & & & & & & & & \\
  %      \hline
   %     Molecule & Transition & S$_\nu\Delta$v$_{TOT}$ & S$_\nu\Delta$v$_{INN}$ & S$_\nu\Delta$v$_{OUT}$ & $\Omega$ & N$_{u~INN}$ & N$_{u~OUT}$ & N$_{u~TOT}$ \\
  %      & & [mJy~km~s$^{-1}$] & [mJy~km~s$^{-1}$] & [mJy~km~s$^{-1}$] & [sr] & [cm$^{-2}$] & [cm$^{-2}$] & [cm$^{-2}$] \\
  %      \hline
  %      & & & & & & & & & \\
  %      p-H$_2$CO & 4$_{2,2}$-3$_{2,1}$ & & & & & & & \\
  %      & & & & & & & & & \\
  %      o-H$_2$CO & 4$_{3,1}$-3$_{3,0}$ & & & & & & & \\
 %       & & & & & & & & & \\
 %       CH$_3$OH-E & 6$_{1,5}$-5$_{1,4}$ & & & & & & & \\
%        & & & & & & & & & \\
 %       \hline
%        \end{tabular}
%\label{table.rotdiagtrans_7}
%\end{table*}
%\noindent Fig. \ref{fig.rotdiag_7} shows the rotational diagrams plotted for the inner and outer disk, as well as the total, for the Cycle 8 methanol transitions shown in Table \ref{table.rotdiagtrans_7}.
%\subsection{Cycle 8}
%\textbf{Thus, the low temperatures measured for both molecules in the outer region} suggests that the dust grains \textbf{here} are icy\textbf{; in contrast,} both molecules are surviving in a warmer reservoir in the inner region. 

%Therefore, we see a decrease in temperature going from the inner to outer region in the emission of both molecules. 
%In this way we obtain separate measurements for both molecules for each emission component of HD 100546: accounting for uncertainties, 
%As can be seen through direct comparison, the measured values for T$_{rot}$ and N$_T$ from analysis of data obtained using GoFish and Specflux are within uncertainty of one another.
%\subsection{Rotational Diagram Analysis}
%\label{Rotational_diagram_analysis}
%As can be seen in Fig. \ref{fig.rotdiag_meth}, there are a handful of outlier points that appear in both rotational diagrams which will therefore not be used to constrain the temperature. The points denoted by triangles are upper limit values (using 5$\sigma$ as a threshold) and are thus too weak to be used - there is one point that is an upper limit value as calculated using both GoFish and Specflux and one that is an upper limit value as calculated by Specflux only; both values are therefore discounted for the temperature constraint especially since the GoFish calculation, while slightly higher than the upper limit value, is still very weak. Meanwhile, the outlier denoted by a star appears to be stronger than expected; this is due to there being two blended CH$_3$OH transitions being represented by this single point (which is necessary due to their having the same E$_u$ value) - this point is also removed from the analysis. 
%Some transitions of CH$_3$OH are omitted completely from the rotational diagram analysis (and thus we do not show their measured opacity in Table \ref{table.rotdiagtrans}): the two CH$_3$OH transitions at 338.513 GHz are, as previously mentioned, completely blended and cannot be separated in frequency, while 
%The CH$_3$OH transitions at 342.730 GHz and 356.007 GHz are, however, excluded from the rotational diagram analysis due to weak s/n of the emission.}% The o-H$_2$CO that are affected by blending in the inner region, on the other hand, are included as they are separated in frequency (291.380 GHz and 291.384 GHz), unlike the blended CH$_3$OH transitions which both appear at 338.513 GHz. Nevertheless, it should be noted that as these two blended transitions therefore appear as a single point on the rotational diagram for H$_2$CO in the inner region. 
%Table \ref{table.rotdiagtrans} shows the S$_\nu\Delta$v values resulting from our extractions in both the inner and outer regions of HD 100546 for both CH$_3$OH and H$_2$CO using the methods as described in Sect. \ref{Methodology}. 
%Also shown in this table are the N$_u$ values calculated from the extracted S$_\nu\Delta$v values using Eq. \ref{eq.nu}. 
%utilising the S$_\nu\Delta$v values shown in Table \ref{table.rotdiagtrans},  
%Also generated are measurements of the opacity for each transition\textbf{, assuming a linewidth calculated using a method first published in \citet{Pegues2020} (see also \citealt{Loomis2018})}; these values are also shown in Table \ref{table.rotdiagtrans}. 
%With all of this taken into account, the resultant plots are shown in Fig. \ref{fig.tempconstrain}. 
%In these plots, we show the best fit gradient and y-intercept for the selected data points, resulting in measurements of T$_{rot}$ and N$_T$, respectively (refer to Eq. \ref{eq.nugu}). 
%We will further discuss the temperature gradient in the disk for both molecules in Sect.~\ref{Rotdiag}. 
%We will compare these ratios with those measured towards other sources, particular the earlier prestellar and protostellar stages that this protoplanetary disk evolved from, in Sect. \ref{Ratios}. 
%We will also discuss our results within the context of astrochemical modelling in Sect. \ref{Modelling}
%\subsection{\ce{CH3OH}/\ce{H2CO} Ratio}
%\label{ratioresults}
%From our rotational diagram analysis, we can compare the column densities of CH$_3$OH and H$_2$CO across different regions of the disk. According to the results for N$_T$ shown in Fig. \ref{fig.tempconstrain}, the total column density measured in H$_2$CO towards HD 100546 is consistent across both regions, as well as being the same order of magnitude that measured in CH$_3$OH towards the outer region; however, the total column density of CH$_3$OH is an order of magnitude higher in the inner region. 
.%is significant and will be discussed further in Sect. \ref{Ratios}.
%\subsection{CH$_3$OH/H$_2$CO ratio}
%As previously mentioned, we can use the GoFish flux extraction to determine the column density of emission detected towards the distinct emission components of CH$_3$OH. According to the moment 0 maps shown in Fig. \ref{fig.morph}, H$_2$CO is also detected in two emission components that are spatially consistent with those traced by CH$_3$OH. As a result of this, we %use the equations presented in Sect. \ref{Methodology} 
%can use our rotational diagram results to calculate the CH$_3$OH/H$_2$CO abundance ratio towards the previously defined inner and outer disk regions. %Due to the weak s/n of the p-H$_2$CO detection, we compute the CH$_3$OH/H$_2$CO ratio using only the o-H$_2$CO emission. In order to account for p-H$_2$CO emission, we assume an ortho-to-para ratio of 3:1 and scale our results for the total extracted flux and column density of H$_2$CO accordingly. %Table \ref{tab.cycle7coldens} shows our results.
%\begin{table*}[hbt!]
%    \centering
%    \caption{Integrated flux densities measured in the inner 110 au using GoFish with a velocity clip between -0.6 and 12.0 km~s$^{-1}$, along with column density values calculated using Eq. \ref{eq.nu} for Cycle 7 CH$_3$OH-E and o-H$_2$CO transitions.}
%    \resizebox{\textwidth}{!}{\begin{tabular}{c c c c c c c}
%        & & & & & & \\
%        \hline
%        Molecule & Transition & Frequency [GHz] & \multicolumn{2}{c}{S$_\nu\Delta$v [mJy km~s$^{-1}$]} & \multicolumn{2}{c}{N$_{u}$ [cm$^{-2}$]} \\
%         \cmidrule(lr){4-5}\cmidrule(lr){6-7}
%        & & & GoFish & Specflux & GoFish & Specflux \\
%        \hline
%        & & & & & & \\
%        CH$_3$OH-E & 6$_{1,5}$-5$_{1,4}$ & 290.249 & 86 $\pm$ 11 & 66 $\pm$ 11 & (8.0 $\pm$ 3.1)$\times$10$^{12}$ & (6.1$ \pm$ 2.4)$\times$10$^{12}$ \\
%        o-H$_2$CO & 4$_{3,1}$-3$_{3,0}$ & 291.384 & 95 $\pm$ 10 & 75 $\pm$ 10 & (2.7 $\pm$ 1.0)$\times$10$^{12}$ & (2.1 $\pm$ 0.8)$\times$10$^{12}$ \\
%        & & & & & & \\
%        \hline
%        \end{tabular}}
%    \label{tab.cycle7coldens}
%\end{table*}
%\newpage 

%As can be seen from our Cycle 7 results, there is consistency within statistical uncertainties between the column density values obtained using GoFish and Specflux. 
%As we are assuming an ortho-to-para ratio of 3:1 in H$_2$CO, w
%We can therefore calculate the total column density of H$_2$CO using the following formula:
%\begin{equation}
%    \rm{N_u(H_2CO})=\Bigg(1+\frac{1}{3}\Bigg)~N_u(\operatorname{o-H_2CO})
%    \label{otp}
%\end{equation}
%This produces a value for the total column density of H$_2$CO as (3.6 $\pm$ 1.3)$\times$10$^{12}$ cm$^{-2}$% measured using GoFish and (2.8 $\pm$ 1.1)$\times$10$^{12}$ cm$^{-2}$ measured using Specflux. 
%Comparing this to our CH$_3$OH values%in Table \ref{tab.cycle7coldens}
%, this produces a CH$_3$OH/H$_2$CO ratio of 2.2$^{+2.6}_{-1.2}$% measured using GoFish and 2.2$^{+2.8}_{-1.9}$ measured using Specflux. 
%low when compared to that measured towards objects of younger evolutionary stages; 
%AN EXAMPLE SENTENCE; THIS POINT MAY BE REMOVED; \textit{It is also important to acknowledge that the H$_2$CO T$_{rot}$ measurements are uniformly lower than those measured for CH$_3$OH. This suggests that there could be a non-LTE factor here, for example, photodesorption or reactive desorption could cause the ice to sublimate in an excited state, which would affect the T$_{rot}$ values measured.} %Similarly, only four out of 11 CH$_3$OH transitions in our sample are detected in the outer region and, once again, the range of E$_u$ values is also small. Therefore, the measurement of further H$_2$CO transitions, especially those of higher E$_u$ values, along with more CH$_3$OH transitions in the outer disk, would be helpful to further constrain the rotational temperature of both CH$_3$OH and H$_2$CO. %Meanwhile, due to the high resolution of our observations, we are probing within the H$_2$O snowline of this object; our CH$_3$OH T$_{rot}$ value measured here is unambiguously lower than that previously found for H$_2$O. 
%Additionally, previous lab-based temperature programmed desorption (TPD) experiments have found that the desorption temperature of pure CH$_3$OH ice is lower than that of H$_2$O-contaminated CH$_3$OH ice by approximately 30 K (\citealt{Collings04}). Therefore, our measurement suggests that methanol ice in this source is pure and there is no mixing with H$_2$O, thus adding strong support to the hypothesis that CH$_3$OH in this source is inherited from an earlier evolutionary stage rather than formed in situ, a conclusion which was first put forward by \citet{Booth2021}. This is because, as illustrated in Fig. \ref{fig.cartoon}, in the inheritance scenario, the pure methanol ice layer frozen out onto the dust grains is preserved from early evolutionary stages, whereas if the methanol has been sublimated during the warmer protostellar phase and then refrozen onto the dust grain as the disk cooled, this methanol ice would have been mixed with water ice as both have very similar binding energies (\citealt{Sandford1988}, \citeyear{Sandford1993}), which would have led to a higher T$_{rot}$ measured in CH$_3$OH in this source than what we actually see.

%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/Cartoon.pdf}
%    \caption{Cartoon illustrating the dust grain ice composition in the scenario where the ice in HD 100546 is inherited from earlier evolutionary stages, thus resembling that of a grain in the ISM (left), compared to the ice composition of a dust grain that has previously been heated to the point of the sublimation of the volatiles shown and subsequently refrozen onto the dust grains as the disk cooled. As illustrated, in the inheritance scenario, the CH$_3$OH is pure and has never been mixed with H$_2$O, unlike in the scenario in which the methanol ice has been sublimated and refrozen at some point in the past, leading to its mixing with H$_2$O. Therefore, the suggestion of a pure rather than mixed CH$_3$OH ice from our low T$_{rot}$ measurement in this source strongly favours the inheritance scenario.}
%    \label{fig.cartoon}
%\end{figure*}

%We also note that the CH$_3$OH column density value found in the present work for HD 100546 is, depending on region, 1-2 orders of magnitude lower than that measured using observations in the present Cycle 8 ALMA Program towards IRS 48 (\citealt{Booth2024IRS}), a similarly warm Herbig disk where CH$_3$OH cannot form in situ. However, an upper limit CH$_3$OH column density that is 2-3 orders of magnitude lower than that measured here towards HD 100546 has been measured towards HD 163296, another Herbig disk, with this measurement being an upper limit due to non-detection of CH$_3$OH, most likely due to the colder temperature of the star leading to freezeout of CO (\citealt{Carney2019}).
%the trend in column density between the inner and outer regions of HD 100546 is inconsistent for our two molecules; 
% which reflects the notion that T Tauri objects are colder environments than Herbig disks. 
%However, the notable decrease going from the inner to the outer disk in both molecules suggests that there are multiple desorption mechanisms at play; the low rotational temperature measured in the outer disk indicates that dust grains are icy here and non-thermal desorption. 
%On the other hand, this work, and the ratio recently measured for HD~169142 ($\approx 20$) by \citep{Booth2023} ar

%The difference in temperature structures between the three Herbig disks HD~100546 and HD~163296 Herbig disks can be attributed to the presences of a cavity in the inner regions of HD~100546 which also leads to a more flared disk which capture
%Furthermore, our results could suggest that there is a higher abundnace of CH$_3$OH compared to H$_2$CO in the ice phase in the disk midplane\textbf{, which is reflected by the thermal ice sublimation in the inner disk}.

%The CH$_3$OH/H$_2$CO abundance ratio found for this source, which is approximately 2.2, is relatively high when compared with other values found in literature.
%The outer region ratio that we derive here is consistent with that obtained by \citet{Booth2021} which assumed either equal rotational temperatures for \ce{CH3OH} and \ce{H2CO} or fixed temperatures of 50 and 30 K, respectively}. 
%\textbf{The right panel of Fig. \ref{fig.tempcomp} shows a comparison between the CH$_3$OH/H$_2$CO ratios measured towards HD 100546 in this work for both the inner and outer regions, along with the aforementioned comparative values towards other Herbig disks, as well as values previously measured towards Class 0, Class I, T Tauri and cometary objects. As illustrated, compared to HD 100546,} slightly higher values of approximately \textbf{2.3$^{+1.1}_{-0.4}$} and an upper limit of 1 have been measured towards disks surrounding T Tauri stars TW Hya (\textbf{\citealt{TerwisschavanScheltinga2021}, Ilee et al. in prep.}) and DG Tau (\citealt{Podio2019}), respectively. It has been suggested that this lower ratio found towards protoplanetary disks surrounding Herbig vs T Tauri stars could be due to low amounts of methanol ice desorption in the midplane due to %shallow geometry,
%differences in the desorption processes present in each type of disk \textbf{(such as photodesorption, x-ray desorption or cosmic-ray desorption)} or due to larger amounts of formaldehyde gas phase production in the upper layers of the Herbig disk (\citealt{Carney2019}). In any case, we note that the CH$_3$OH upper limit column density measured towards HD 163296 is two orders of magnitude less than that found towards HD 100546, which suggests that the difference in ratio could be attributed to something affecting CH$_3$OH rather than H$_2$CO abundance\textbf{, although the detection of CH$_3$OH in HD 100546 does not support these differences.
%Taking this, along with the large uncertainty associated with our ratio, into account, the abundance ratio towards HD 100546 is much closer numerically with Class I/II than Class 0 objects and may even be consistent with the former.
%\subsection{Methanol Binding Energy}\label{binding_energies}
%As a result of constraining the rotational temperature of methanol, we are able to also constrain its binding energy in this environment. In order to achieve this, we use a method similar to that used by \citet{vantHoff2017} to study CO in TW Hya; we invert this method such that the binding energy of CH$_3$OH is obtained by assuming that we are at or close to the CH$_3$OH snowline due to the value of our constrained rotational temperature and thus we assume that the ratio between ice and gas phase methanol at this location (and thus the ratio of the rate coefficients of freeze-out and desorption) is approximately 1:1. This results in the derivation of Eq. \ref{eq.dali}; please see the Appendix for a full explanation of the methodology and derivation of this equation.
%\begin{equation}
%    E_b=T_dln\Bigg(\frac{\nu_0}{\sqrt{\frac{8k_BT_g}{\pi m}}\sigma_{grain}n_{grain}}\Bigg)
%    \label{eq.dali}
%\end{equation}
%In Eq. \ref{eq.dali}, E$_b$ represents the binding energy of CH$_3$OH (K), T$_d$ represents the dust temperature (K), $\nu_0$ represents the characteristic vibrational frequency of an adsorbed species in its potential well (s$^{-1}$), k$_B$ represents the Boltzmann constant in its cgs units, T$_g$ represents the gas temperature (K), m represents the mass of the molecule (g), $\sigma_{grain}$ represents the cross section of the dust grain (cm$^{-2}$), n$_{grain}$ represents the number density of the dust grains (cm$^{-3}$ and S represents the sticking coefficient (assumed in this case to be 1). As we are under the LTE assumption, T$_d$ is assumed to be equal to T$_g$ and is given by the value of T$_{rot}$ found in the present work, which is approximately 90 K in the inner region that we are considering. We assume a constant v$_0$ of 10$^{-12}$ s$^{-1}$ and calculate the mass assuming a molar mass for CH$_3$OH of 32.04 g~mol$^{-1}$. For the rest of the parameters, we use the results of applying the 2D physical chemical code DALI (refer to \citealt{Bruderer2012} for further details) to HD 100546 (Leemker et al. in prep.) at the radial distance where the temperature is within uncertainty of our results: a temperature of 96.171 K is found at approximately 20 au. This radial distance corresponds approximately to the location of the inner cavity wall (\citealt{Pineda2019}) and at this distance, the other physical parameters are shown in Table \ref{tab.dali}. Finally, cross sectional area ($\sigma$) is calculated for both large and small dust grains; according to Leemker et al. (in prep.), small dust grains have an assumed radius between 5 nm and 1 $\mu$m while large dust grains are assumed to have radii between 5 nm and 1 mm. The full methodology for calculating cross sectional area can also be found in the Appendix.
%\begin{table}[hbt!]
%    \centering
%    \caption{Physical parameters obtained by applying the DALI model to HD 100546 at a radial distance of approximately 20 au.}
%    \begin{tabular}{c c c}
%    \hline
%         Parameter & Value & Units \\
%         \hline
%        T$_d$ & 96.171 & K \\
%        T$_g$ & 96.171 & K \\
%        n$_{grain}$ & 5.41$\times$10$^{10}$ & cm$^{-3}$ \\
%        \hline
%    \end{tabular}
%    \label{tab.dali}
%\end{table}
%\\
%\\
%Taking into account the range of dust grain sizes, we obtain binding energy values ranging from 3148 to 3678 K. This is notably smaller than the binding energy found for pure CH$_3$OH - a value of 4235 $\pm$ 15 K (\citealt{Sandford1993}, \citealt{Cuppen2017}).
%suggest the presence of multiple radially separated desorption mechanisms in this disk, which would give rise to differing chemical environments in regions in which planet formation is underway (\citealt{Quanz2013}, \citealt{Walsh2014}, \citealt{Brittain2014}). 
%Therefore, we also supplement our observations with chemical modelling; we utilise a gas-grain chemical model first published in \citet{Walsh2010} to investigate the presence of both CH$_3$OH and H$_2$CO towards HD 100546.
%it seems that at the radii that we are investigating with our data, ranging from 110-260 au, the model is predicting a column density of CH$_3$OH that is two orders of magnitude lower than that observed in the inner region and one order of magnitude lower than that seen in the outer region. Consequently, the model does not predict the observed order of magnitude decrease in gas-phase CH$_3$OH that is seen in our observations. On the other hand, a decrease in the gas-phase H$_2$CO column density of an order of magnitude from 10$^{13}$ to 10$^{12}$ cm$^{-2}$ is predicted by the model but not seen in the observations, where the value stays approximately constant at 10$^{13}$ cm$^{-2}$. As a result of these trends, there is a discrepancy between the CH$_3$OH/H$_2$CO ratio predicted by the model vs observations, with the model predicting a higher ratio in the }
%\\
%\\
%\textit{Include description and discussion of different desorption mechanisms in this section.}
%, although both clearly peak around the previously observed dust ring at approximately 200 au (\citealt{Pineda2019})

%By comparing between the observational column densities obtained through our observational results (refer to the rotational diagrams in Fig. \ref{fig.tempconstrain}) and the column densities predicted by the model in Fig. \ref{fig.ncol_model}, it seems that the overall trends for both CH$_3$OH and H$_2$CO from the inner to the outer \textbf{disk} are very comparable. 

%More specifically, . This is in line with our observational results, which show a marked decline in CH$_3$OH/H$_2$CO ratio from the inner to outer \textbf{disk} from $\sim$15 to $\sim$1, a consequence of the order of magnitude decrease in CH$_3$OH column density. \textbf{To further illustrate this, in Fig. \ref{fig.modellingratio}, we show how the same gas-grain model predicts the trend of the CH$_3$OH/H$_2$CO ratio in HD 100546 with radius, again for time periods of 1, 2 and 5 Myr.} This is further evidence for the existence of multiple radially separated desorption mechanisms, hence strengthening our suggestion that there are multiple chemical environments in this planet-forming disk.
%approximately 110 au and, in H$_2$CO and, in four CH$_3$OH lines, emission corresponding with the previously detected dust ring at approximately 200 au, enabling us to run separate analyses for both regions of the disk for each molecule.
   %low compared to values seen towards objects in earlier stages of low mass stellar evolution, suggesting that the gas phase methanol being detected has been sublimated from pure methanol ice and is therefore only now seeing the gas phase for the first time, rather than from ice that is water-contaminated due to previous sublimation of volatiles including methanol and water from the dust grain surface and subsequent refreezing as a mixed ice due to their similar binding energies. Our results therefore strongly support the suggestion that methanol in HD 100546 is indeed inherited from previous evolutionary stages
%Using our obtained value for the rotational temperature of CH$_3$OH at the approximate location of the inner dust cavity wall at 20 au, along with DALI modelling results for HD 100546, we calculate the binding energy of CH$_3$OH in this environment to range from 3148 to 3678 K, depending on the dust grain size, for which we adopt a range according to previous modelling assumptions. This is notably lower than the previously obtained binding energy for CH$_3$OH according to TPD experiments involving pure CH$_3$OH ice.
% With in situ formation impossible, the logical explanation was that methanol in these sources has been inherited from previous evolutionary stages. Building upon this, we have clearly detected 10 CH$_3$OH lines and five H$_2$CO lines towards HD 100546, enabling us to constrain the rotational temperature of both molecules within the water snowline of this source to temperatures in agreement with thermal desorption, albeit with different desorption mechanisms clearly at play in different spatial regions of this disk%, giving rise to a spatial variation in the rotational temperature of methanol. While the temperatures measured are too high to strongly suggest inheritance of CH$_3$OH in HD 100546, we can conclude even from our observations prior to analysis that there is a clear presence of the simplest COM towards this Herbig disk, which is in itself not guaranteed; %90 K, a value lower than that of water. This, along with evidence from TPD experiments, suggests that the methanol ice in this source is pure and has never been mixed with water ice, strongly supporting the methanol heritability argument. However, this argument does not apply to all Herbig disks; methanol was not detected towards %MWC 480, CQ Tau or for example, in the case of HD 163296 (%\citealt{Oberg2010}, \citealt{Carney2019}), the colder temperature gives rise to CO freezeout suggesting that any methanol present is not in the detectable gas phase. 
%}, it seems that CH$_3$OH is detected (and therefore potentially inherited) only in some Herbig disks. It is, however, unclear due to a lack of sample size of observations towards Herbig disks whether this difference exists as a full dichotomy or as more of a gradient between scenarios; 
%have major implications on the study of our own origins.%\begin{figure*}[hbt!]
 %   \centering
  %  \includegraphics[width=0.35\textwidth]{images/H2CO_cold_mom0.png}
   % \includegraphics[width=0.35\textwidth]{images/H2CO_mid_mom0.png}
    %\includegraphics[width=0.35\textwidth]{images/H2CO_extra_mom0.png}
    %\includegraphics[width=0.35\textwidth]{images/H2CO_hot_mom0.png}
    %\caption{Moment 0 maps for all H$_2$CO transitions used in the flux extraction and rotational diagram analysis, in ascending order of E$_u$. The top-right panel is the line at 291.384 GHz and the bottom left panel is the line at 291.380 GHz; both have identical E$_u$ values. Note that two blended o-H$_2$CO lines are present in the rightmost panel. The synthesised beam is represented by the white ellipse in the lower left corner.}
    %\label{fig.mom0_h2co}
%\end{figure*}
%    However, the temperature towards the outer region of HD 100546 is much lower compared to the younger objects, again reinforcing the conclusion that two separate chemical environments are present in the two regions of \textbf{the} HD 100546 \textbf{disk}. However, we note that our sample size is small, especially with regard to Class II objects with this being the first study to detect enough \ce{CH3OH] lines to constrain the rotational temperature towards one. 
%With methanol being vital to the formation of life-sustaining molecules, increasing our understanding of its behaviour and presence, in particular in planet-forming regions of disks, could \textbf{shed light on the availability of pre-biotic molecules and their precursors during planet formation in objects in the local galaxy.} 
%\begin{figure*}[hbt!]
%    \centering
%    \includegraphics[width=0.95\textwidth]{images/specflux_wide.png}
%    \caption{CH$_3$OH emission spectra showing flux extracted using Specflux between 0 and 110 au for the full velocity range of the spw (-4.2 and 17.4 km~s$^{-1}$) used to check the suitability of GoFish for our data, where some lines are unresolved in the inner region. The grey dashed line indicates the source velocity at 5.7 km~s$^{-1}$.}
%    \label{fig.specflux_wide}
%\end{figure*}
%(excluding the line at 350.688 GHz due to its blending with a non-CH$_3$OH line)
%\section{Channel Maps}
%Figs. \ref{fig.firstchan7} to \ref{fig.lastchan7} show the channel maps for Cycle 7 data, showing CH$_3$OH, p-H$_2$CO and o-H$_2$CO detections. Figs. \ref{fig.firstchan} to \ref{fig.lastchan} show the channel maps for the full spws targeted for all 12 CH$_3$OH lines, in descending order of peak intensity. Fig. \ref{fig.stackedchan} shows the channel map generated by stacking the individual spw channel maps of the CH$_3$OH lines in our Cycle 8 sample.
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_1_channels_c7.png}
%    \caption{Channel map showing the CH$_3$OH emission seen in our Cycle 7 observations. The synthesised beam is represented by the white ellipse in the lower left corner.}
%    \label{fig.firstchan7}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_2_channels_c7.png}
%    \caption{Channel map showing the p-H$_2$CO emission seen in our Cycle 7 observations. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_3_channels_c7.png}
%    \caption{Channel map showing the o-H$_2$CO emission seen in our Cycle 7 observations. The synthesised beam is represented by the white ellipse in the lower left corner.}
%    \label{fig.lastchan7}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_1_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 338.408 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%    \label{fig.firstchan}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_2_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 338.614 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_3_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 338.345 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_4_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 338.513 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_5_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 338.124 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_6_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 338.560 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_7_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 338.640 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_8_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 350.688 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_9_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 349.107 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_10_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 342.730 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_11_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 356.007 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \includegraphics[width=\textwidth]{images/line_12_channels.png}
%    \caption{Channel map showing CH$_3$OH line at 355.603 GHz. The synthesised beam is represented by the white ellipse in the lower left corner.}
%    \label{fig.lastchan}
%\end{figure*}
%\begin{figure*}[hbt!]
%    \centering
%    \includegraphics[width=\textwidth]{images/Cycle8_stacked_channels.png}
%    \caption{Channel map created by stacking the channel maps for the 12 CH$_3$OH lines detected in our Cycle 8 observations (see Fig. \ref{fig.firstchan} to \ref{fig.lastchan}). The synthesised beam is represented by the white ellipse in the lower left corner.}
%    \label{fig.stackedchan}
%\end{figure*}
%\newpage
%\newpage
%\section{Binding Energy Methodology}
%In Section \ref{binding_energies} we introduce the equation derived using elements of the methodology from \citet{vantHoff2017} to calculate the binding energy of methanol in HD 100546 at around the location of the inner cavity wall. Here, we describe in full the derivation of Eq. \ref{eq.dali} and explain our assumptions.
%\\
%\\
%According to \citet{vantHoff2017}, freeze out and desorption rates of a species can be described using the following relation:
%\begin{equation}
%    k_dn_s=k_fn_g,
%    \label{eq.a.1}
%\end{equation}
%with k$_d$ and k$_f$ representing the rates of desorption and freeze out, respectively, while n$_s$ and n$_g$ represent the number density values of the species in the solid (ice) and gas phase, respectively, both in units of cm$^{-3}$. Our derived T$_{rot}$ for CH$_3$OH suggests that we are at or close to the snowline in this source, which means that the ratio of CH$_3$OH in the ice:gas phase is approximately 1:1. This enables us to assume that the number densities (n$_s$ and n$_g$) in this case are equal and thus the reaction rates of desorption and freeze out, k$_d$ and k$_f$, are also equal.
%\\
%\\
%In particular, these reaction rates can be calculated using the following formulae:
%\begin{equation}
%    k_d=\nu_0e^{-\frac{E_b}{T_d}}
%    \label{eq.kd}
%\end{equation}
%\begin{equation}
%    k_f=\textless \rm{v} \textgreater \sigma_{grain}n_{grain},
%    \label{eq.kf}
%\end{equation}
%in which $\nu_0$ is the characteristic vibrational frequency of an adsorbed species in its potential well, which we assume to be constant, E$_b$ is our binding energy, T$_d$ is our dust temperature, $\textless$v$\textgreater$ is the thermal velocity of a mass m of molecules at a gas temperature T$_g$, $\sigma_{grain}$ is the average cross section of the dust grains and n$_{grain}$ is the number density of the dust grains. Within Eq. \ref{eq.kf}, $\textless$v$\textgreater$ is given by:
%\begin{equation}
%    \textless \rm{v} \textgreater = \sqrt{\frac{8k_BT_g}{\pi m}},
%    \label{eq.thermalvelocity}
%\end{equation}
%where k$_B$ is the Boltzmann constant. Meanwhile, we calculate $\sigma$ for both large and small dust grains, assuming a radial range (a) of 5 nm to 1 mm for large dust grains and 5 nm to 1 $\mu$m for small dust grains. We also assume a constant gas:dust bulk density ratio of 100; all of these values are taken from the modelling work of Leemker et al. (in prep.). We calculate the bulk gas density, $\rho_{gas}$, assuming a number density of 10$^{12}$ cm$^{-3}$ in the gas phase and use our assumed constant ratio to calculate the bulk dust grain density, $\rho_{dust}$. We also assume that a power law with an exponent of -3.5 describes number density as a function of radius, a, such that:
%\begin{equation}
%    \frac{dn}{da}=xa^{-3.5},
%    \label{eq.powerlaw}
%\end{equation}
%where x is a constant scale factor. By writing $\rho_{dust}$ in terms of number density, n$_{dust}$:
%\begin{equation}
%    \rho_{dust}=\frac{n_{dust}V}{\rho_{dust}},
%    \label{eq.definition}
%\end{equation}
%where V is the spherical volume given by:
%\begin{equation}
%    V_{sphere}=\frac{4}{3}\pi a^3,
%    \label{eq.sphericalvolume}
%\end{equation}
%we can therefore use Eq. \ref{eq.powerlaw} to write an equation to describe bulk dust grain density, $\rho_{dust}$:
%\begin{equation}
%    \rho_{dust}=\int^{a_{max}}_{a_{min}}\frac{4}{3}\frac{np.pi}{\rho}xa^{-3.5}a^3da.
%    \label{eq.densities}
%\end{equation}
%Rearranging, we can write an equation for the scaling constant of Eq. \ref{eq.powerlaw}, x:
%\begin{equation}
%    x=\Bigg(\int^{a_{max}}_{a_{min}}\frac{4}{3}\frac{\pi}{\rho_{dust}^2}a^{-0.5}\Bigg)^{-1}
%    \label{eq.x}
%\end{equation}
%Using our resultant values for x in the separate cases of large and small dust grains, along with Eq. \ref{eq.powerlaw}, we can use the following equation to calculate grain cross sectional area, $\sigma_{grain}$:
%\begin{equation}
%    \sigma_{grain}=\int^{a_{max}}_{a_{min}}\pi a^{2}xa^{-3.5}da.
%    \label{eq.sigma}
%\end{equation}
%We obtain results for $\sigma_{grain}$ ranging from 1.2 $\times$10$^{12}$ cm$^{-2}$ for the small dust grains to 3.0 $\times$10$^{-10}$ for the large dust grains.
%\\
%\\
%By inserting Eq. \ref{eq.thermalvelocity} into Eq. \ref{eq.kf} and in turn equating Eqs. \ref{eq.kd} and \ref{eq.kf} using Eq. \ref{eq.a.1} and our assumption that n$_s$ and n$_g$ are equal, rearranging for E$_b$ yields Eq. \ref{eq.daliappendix}, which is used in our calculation in Sect. \ref{binding_energies}.
%\begin{equation}
%    E_b=T_dln\Bigg(\frac{\nu_0}{\sqrt{\frac{8k_Bt_g}{\pi m}}\sigma_{grain}n_{grain}}\Bigg)
%    \label{eq.daliappendix}
%\end{equation}
%It should be noted that the former value leads to a small discrepancy when comparing obtained column density values \textbf{with those obtained by \citet{Booth2024HD}, however, those results were obtained using the peak flux of only one CH$_3$OH transition and assuming the emitting area as the beamsize of their observations}. 

